Cronus: Robust and Heterogeneous Collaborative Learning with Black-Box Knowledge Transfer

Collaborative (federated) learning enables multiple parties to train a model without sharing their private data, but through repeated sharing of the parameters of their local models. Despite its advantages, this approach has many known privacy and security weaknesses and performance overhead, in addition to being limited only to models with homogeneous architectures. Shared parameters leak a significant amount of information about the local (and supposedly private) datasets. Besides, federated learning is severely vulnerable to poisoning attacks, where some participants can adversarially influence the aggregate parameters. Large models, with high dimensional parameter vectors, are in particular highly susceptible to privacy and security attacks: curse of dimensionality in federated learning. We argue that sharing parameters is the most naive way of information exchange in collaborative learning, as they open all the internal state of the model to inference attacks, and maximize the model's malleability by stealthy poisoning attacks. We propose Cronus, a robust collaborative machine learning framework. The simple yet effective idea behind designing Cronus is to control, unify, and significantly reduce the dimensions of the exchanged information between parties, through robust knowledge transfer between their black-box local models. We evaluate all existing federated learning algorithms against poisoning attacks, and we show that Cronus is the only secure method, due to its tight robustness guarantee. Treating local models as black-box, reduces the information leakage through models, and enables us using existing privacy-preserving algorithms that mitigate the risk of information leakage through the model's output (predictions). Cronus also has a significantly lower sample complexity, compared to federated learning, which does not bind its security to the number of participants.

==> algorithm.tex <==
\section{Preliminaries}



\subsection{Federated Learning Framework}\label{fed_learn}

McMahan et al. \cite{mcmahan2016communication} proposed a federated learning algorithm.
In each round, $N$  collaborating clients learn models  $\theta_i$ locally, e.g. by updating the model multiple times using SGD steps, and then share the knowledge $U_i$ with a central server.
The server then aggregates the knowledge $U_i$ using the average algorithm and send the aggregated result $U_{agg}$ to the local clients. The two processes are described in the Algorithm ~\ref{alg:fed}.

\begin{algorithm}
\caption{Federated Learning Framework}
\label{alg:fed}
\begin{algorithmic}[1]
\Procedure {\textsf{\small{ClientOp}}}{$U_{agg}$}
\State $U_i$ $\leftarrow$ update $U_i$ based on $U_{agg}$ and local private dataset $D_{i}$
\State return $U_i$ to server
\EndProcedure

\Procedure {\textsf{\small{ServerOp}}}{$U_1,U_2,...,U_N$}
\State $U_{agg} = f_\textsf{\tiny{AGG}}(U_1,U_2,...,U_N)$
\State Return $U_{agg}$ to local clients
\EndProcedure
\end{algorithmic}
\end{algorithm}

\red{\subsection{Byzantine Problem}
In federated learning, some of the clients can be an adversary and share the arbitrary knowledge to destroy the aggregated result.
In this paper, let $N$ is the number of local clients, and the $M$ of them possibly Byzantine workers.Let d is the size of the model gradient or parameter}


\section{Aggregation Schemes}\label{aggregation}
For federated learning, in most of the case, the knowledge of the local clients are represented via the local model gradient or the local parameter.
The vanilla federate learning uses an aggregation based on the simple averaging which we will discuss in this section.
However, the simple averaging is susceptible to the simple poisoning attacks, e.g. when all the $M$ malicious clients learn local models on the data whose labels are changed \ref{attack:lf_poison}.
Different aggregation schemes are proposed in the literature to mitigate simple and advanced poisoning attacks on collaborative learning schemes. Below, we detail robust averaging schemes.





\subsection{Vanilla Aggregation}
In the vanilla federate learning, the server computes a weighted average of client knowledge where weights are assigned based on the size of local training data of each client. Here is the knowledge is the model parameter $\theta_i$.
Specifically, the server averages parameters of all the client models $\theta_i$, to get a aggregated result $\theta_{agg} = \sum^N_{i=1}\frac{|D_i|}{|D|}\theta_i$.
Here $|D_i|$ is the size of local training data of $i^{th}$ client and $|D|=\sum^N_{i=1}|D_i|$.




\subsection{Krum}\label{aggregation:krum}
As we discussed at the beginning of this section, the simple averaging algorithm can be very vulnerable. To solve this problem, Blanchard et al. \cite{blanchard2017machine} proposed Krum aggregation. The sharing knowledge of the Krum is the model gradient.
The intuition behind Krum is that in a normal distribution, the vector with average parameters in each dimension will be the closest to all the parameters vectors drawn from the same distribution. So instead of calculate the average of the vectors, the Krum find the points which are closest to every vector. However, since the dataset contains bad vector which can be arbitrarily large. So Krum only considers the distance to the closest $N-M-2$ clients, sets of parameters which will differ significantly from the average vector are outliers and will be filtered.
The detail is as below:
Let $\theta_1,...,\theta_N$ be the received.
For $i\neq j$, let $i \rightarrow j$ denote the fact that $\theta_j$ belongs to the $N-M-2$ updates closest to $\theta_i$.
Finally, let $s(\theta_i) = \sum_{i \rightarrow j} ||\theta_i-\theta_j||^2$ be the \emph{score} of $\theta_i$.
Then, Krum outputs the $\theta_k$ with the lowest score.
This is formalized in \eqref{krum}.


\begin{equation}\label{krum}
f_\textsf{\tiny{AGG\_Krum}}(\theta_1,...,\theta_N) = \Bigg(\theta_k\big| \underset{k\in[N]}{\text{argmin}} \sum_{i \rightarrow j} ||\theta_i-\theta_j||^2 \Bigg)
\end{equation}



\subsection{Bulyan}\label{aggregation:bulyan}


Krum was proved to be $(\alpha-M)$\emph{-Byzantine tolerant}, i.e. it can tolerate up to $M$ malicious clients such that $N>2M+2$.

However, El Mhamdi et al. \cite{mhamdi2018the} proposed an attack on Krum.
The omniscient adversary perturbs the value only of a single dimension of $\theta_i$ by an arbitrarily large amount and keeps the value of all other dimensions at the average of values of benign updates.
This does not affect the $L^p$ norm of the distance between $\theta_i$ and $\theta_k$ but affects the convergence of Krum.
They show that the convergence alone should not be the target, because parameters can converge to an ineffective model.


El Mhamdi et al. \cite{mhamdi2018the} propose \emph{Bulyan}, a meta-aggregation rule, which takes another aggregation rule, $\mathcal{A}$, as an additional input.
At first, Bulyan is using $\mathcal{A}$ iteratively to create a SelectionSet of probably benign candidates,
and then aggregates this set by the second variant of TrimmedMean.
Bulyan combines methods working with $L^p$ norm that proved to converge, with the advantages of methods working on each dimension separately, such as TrimmedMean, overcoming Krum’s disadvantage described above because TrimmedMean will not let the single malicious dimension slip.
Algorithm \ref{alg:bulyan} describes the aggregation.
% It should be noted that on line 6, n��4m values are being averaged, which is n0��2m for n0 = jSelectionSetj = n �� 2m.

\begin{algorithm}
\caption{Bulyan aggregation: $f_\textsf{\tiny{AGG\_Bulyan}}$ \cite{mhamdi2018the}}

\label{alg:bulyan}
\begin{algorithmic}[1]
\State \textbf{Input}: $\mathcal{A}$, $\mathcal{P}=(\theta_1,...,\theta_N)$, $N$,$M$
\State $S\leftarrow \emptyset$
\While{$|S|<N-2M$}
	\State $p \leftarrow \mathcal{A}(\mathcal{P}\backslash $S$)$
	\State $S\leftarrow S\cup \{p\}$
\EndWhile
\State \textbf{Output}: $TrimmedMean(S)$
\end{algorithmic}
\end{algorithm}

$TrimmedMean$ clusters $N-M$ values closest to the \emph{median} of all the values of $j-{th}$ dimension of all the $\theta_i$'s and assigns mean of the $N-M$ values to $\theta_j$.
Assuming all $\theta$ are $d$-dimensional, $TrimmedMean$ is given by \eqref{trimmed_mean}.

\begin{equation}\label{trimmed_mean}
TrimmedMean(\theta_1,...,\theta_N) =\Bigg\{\theta^j=\frac{1}{|U_j|} \sum_{i\in U^j} \theta_i^j \ \forall j\in [d]  \Bigg\}
\end{equation}


There are different variants of $TrimmedMean$ \cite{xie2018generalized,mhamdi2018the,yin2018byzantine}, but we follow the one used in \cite{mhamdi2018the}.
Hence, in \eqref{trimmed_mean}, $U_j$ is the set of the indices of top-$N-2M$ values in $(\theta_1^j,...,\theta_N^j)$ nearest to their median $\mu_j$.
% Hence, note that at line 6 of Algorithm. \ref{alg:bulyan}, $N-4M$ are being averaged.
% Bulyan is designed to defend against $(\frac{N-3}{4})$ malicious clients.










\subsection{Multiplicative weight update}\label{aggregation:mwu}

Krum and Bulyan aggregation rules are specifically designed to aggregate gradients or parameter updates.
Therefore, the analysis of the utility of the aggregated model obtained in the end is based on the convergence of the model.
Both Krum \cite{mhamdi2018the} and Bulyan \cite{baruch2019a} are shown to be susceptible to attacks by the strong adversary that we consider in our work.
Next, we consider \emph{robust mean estimation algorithms}, that aim to estimate the mean of $d$-dimensional data.
These algorithms assume that among $N$ data points, $\epsilon$ fraction of data points are drawn from some \emph{random} distribution while rest of the points are drawn from some distribution $P$ whose mean is to be estimated.



The first algorithm we consider is \emph{multiplicative weight update} (MWU).
MWU is a simple technique that lies at the core of many algorithms\cite{arora2012the,freud1997decision,plotkin1991fast,garg2007faster,li2014resolving}.
Li et al. \cite{li2014resolving} propose a truth discovery algorithm, \emph{CRH framework}, that uses MWU technique to reduce the weight of unreliable clients and increase that of reliable clients based on the distance of their response from a function, e.g. average or median, of all the responses.
The general framework of MWU is given in Algorithm. \ref{alg:mwu}.
The intuition behind MWU based defenses is to reduce the weights of malicious clients assuming that they lie farther away from the mean than the benign clients.
Therefore, MWU based aggregation schemes are designed to handle up to $\floor{\frac{N-1}{2}}$ malicious clients.
There are different variants of MWU that use different functions for $\textsc{WeightUpdate}$ and $f_\textsf{\tiny{AGG}}$.
We detail these next.


\begin{algorithm}
\caption{Multiplicative weights update}
\label{alg:mwu}
\begin{algorithmic}[1]
\State \textbf{Input}: $\mathcal{P}=(\theta_1,...,\theta_N)$
\State Initialize aggregate $\theta^{t=0}$, client weights $\mathbf{w}^0$, $t=0$

\Repeat

	\State $\mathbf{w}^{t+1}\leftarrow$ \textsc{{WeightUpdate}} ($\theta^t$, $\theta_{i,i\in [N]}$)
	% \Comment {Update client weights}

	\State $\theta^{t+1} \leftarrow f_\textsf{\tiny{AGG}}(\theta_{i,i\in [N]}, \mathbf{w}^{t+1})$
	% \Comment {Update aggregate}

	\State $t=t+1$

\Until {Convergence criterion is satisfied}

\State \textbf{Output}: $\theta^T$, $\mathbf{w}$
\end{algorithmic}
\end{algorithm}


\subsubsection{MWU with average}


In MWU with average (\emph{MwuAverage}), weight update is based on distance between the aggregate, $\theta$, and the individual $\theta_i$; this is given by \eqref{mwu_avg_wu}.
Note that, Krum and Bulyan handle each dimension of $\theta_i$ separately, but MWU handles the entire $d$-dimensional update vector, $\theta_i$, at once.

\begin{align}
\label{mwu_avg_wu}
w^{t+1}_i &= w^{t}_i \text{exp}(- ||\theta-\theta_i||_p)\\
\label{mwu_avg_agg}
\theta &= \sum^N_{i=1}w_i \theta_i
\end{align}


Similar to the MwuAverage, MWU with median (\emph{MwuMedian}) is defined.
In MwuMedian, instead of computing weighted average as the aggregate in each round, weighted median is computed.
In both the aggregation, MwuAverage and MwuMedian, convergence criterion is satisfied when $\theta^{t+1}$ does not change significantly from $\theta^{t}$, i.e. $|\theta^{t+1}-\theta^{t}| < \epsilon$.
Another way to impose this condition is to run MWU algorithm for $T$ iterations and output $\theta^{T}$.
MwuAverage works well against some of the attacks that are proposed in the literature \cite{baruch2019a,mhamdi2018the}.
We design an attack (Section. \ref{attack:attack_on_averaging}) that completely jeopardizes the accuracy of models trained using \emph{any} aggregation scheme that involves averaging.
Similar to Bulyan, MwuMedian is susceptible to the attack proposed in \cite{baruch2019a}.


\subsubsection{MWU based on optimization}

Li et al. \cite{li2014resolving} propose CRH framework for truth discoverty from crowd-sourced data.
In each epoch, the framework updates the weights of clients based on solution of an optimization.
Essentially, the weight update considers the distance of update of client from the aggregate of all the updates in the epoch.
The weight and aggregate updates are given by \eqref{mwu_opt_wu} and \eqref{mwu_opt_agg}, respectively.
For details of the optimization, please refer to \cite{li2014resolving}.


\begin{align}
\label{mwu_opt_wu}
w^{t+1}_i &=-\text{log}\Bigg(\frac{||\theta-\theta_i||_p}{\sum^N_{i=1}||\theta-\theta_i||_p}\Bigg)\\
\label{mwu_opt_agg}
\theta &= \sum^N_{i=1}w_i \theta_i
\end{align}

\subsection{High dimensional Robust Mean Estimation}
The MWU is trying to solve the mean estimation by increasing the weight to the benign points and reducing the weight of the bad clients.
In the robust statistics, there are lots of different technics to build a robust mean estimator. However, similar to the limitation of the related work, the high dimension still remains hardness in the robust statistics area. The problems with robustness in high dimension would be Computationally intractable and Statistically suboptimal. In the federated learning setting, the dataset dimension should not be the bottleneck of the framework. In other words, the aggregation algorithm should not be affected by the dimension of the input in terms of the robustness in the federate learning settings.


Based on this intuition, we aim to find the robust mean estimation which preserved robustness in the high dimensional dataset.  Recently, there are some works propose the robust mean estimation in the high dimension. In the work \cite{steinhardt2018robust}, the author proposed robust mean estimation via moments and eigenvectors.


\begin{theorem}\cite{steinhardt2018robust}
Suppose that $x_1,...,x_n \in \mathbb{R}^d$ contain a subset S of size $(1 - \epsilon)n$ that has bounded covariance: $\frac{1}{|S|} \sum_{i \in S}(x_i - \mu)(x_i - \mu)^T \preceq \sigma^2 I$,where $\mu$ is the mean of S. Then if $\epsilon \leq \frac{1}{12}$, there is an efficient algorithm (Algorithm ~\ref{alg:filterL2}) whose output $\hat{\mu}$ satisfies $||\hat{\mu} - \mu||_2 = o(\sigma\sqrt{\epsilon})$
\end{theorem}


\begin{algorithm}
\caption{FilterL2 \cite{steinhardt2018robust}}
\label{alg:filterL2}
\begin{algorithmic}[1]

\State \textbf{Input}: $x_1,...,x_n \in \mathbb{R}^d$
\State Initialize weights $c_1,...,c_n =1.$
\State Compute the empirical mean $\hat{\mu}$ of the data, $\hat{\mu} = (\sum_{i=1}^n c_i x_i)/(\sum_{i=1}^n c_i)$
\State Compute the empirical covariance $\hat{\Sigma} = \sum_{i=1}^n c_i(x_i -\hat{\mu})(x_i - \hat{\mu})^T /\sum_{i=1}^n c_i $


\State Let $v$ be the maximum eigenvector of $\hat{\Sigma}$ and let $\hat{\sigma}^2 = v^T\hat{\Sigma}v$

\State If $\hat{\sigma}^2\leq 16 \sigma^2$,output $\hat{\mu}$
\State Otherwise,let $\tau_i = <x_i  - \hat{\mu},v>^2$ \State Update $c_i \leftarrow c_i \dot (1-\tau_i/\tau_{max})$,where $\tau_{max} = \max_i \tau_i$
\State Go back to line 3
\end{algorithmic}
\end{algorithm}

The algorithm is proposed for the high dimensional dataset which error guarantee is independent of the dimension. In federated learning, this weight update process is happening in each iteration. Then the convergence speed of the weight can be one of the bottlenecks. Meanwhile, we assignment the weight to each clients knowledge. The limitation here is similar to the MUW with averaging. The attack may first put few adversarial points extremely far away from the real mean. Initially, all the points have the same weight which is 1. The empirical mean will be far away from the real mean. In this case, the distance between the normal points to the empirical mean is large. The small weight will assign to normal points. At the same time, if the adversary would put some adversarial points near the destroyed empirical mean, then the larger weight will assign to the adversarial points. We design attack which is targeted to this weight assigned method in the Section ~\ref{attack:attack_on_averaging}



\red{The analysis of the Table ~\ref{tab:theory_analysis} shows that the statistical error rate of aggregation schema proposed in the related work actually depends on the dimension of the input. In most of the case, the input is the model parameter or the gradient which is extremely large for the large deep learning model. For the cronus, we not only reduce the dimension of the data but also remove the dependency of the error guarantee to the dimension.}


\begin{table*}
\fontsize{8}{11}\selectfont{}
\begin{center}
\begin{tabular}{|l|c|c|c|c|}
\hline
& \multicolumn{1}{l|}{Byzantine Fraction}
&\multicolumn{1}{l|}{Statistical Error Rate}
& \multicolumn{1}{l|}{Computational Complexity}
& \multicolumn{1}{l|}{Sample Complexity} \\
\hline Mean
& 0
& *
& *
& * \\
\hline Median
& $\alpha < 1/2 $
& $\Theta(\alpha\sqrt d)$
& $O(Nd\log N )$
& * \\
\hline Krumm
& $\alpha < 1/2 - 1/N$
& $O(N\sqrt{d} \sigma)$
& $O(N^2 d)$
& * \\
\hline Bulyan
& $\alpha \textless 1/4 - 3/(4N)$
& $O(\sqrt{d} \sigma)$
& $O(N^2 d + Nd) $
& * \\
\hline
Cornus
& *
& $O(\alpha \sqrt{1/\alpha})$
& $O(d_p^2 + d_p^3 + N)$
& $\Omega((d_p/\alpha^2)) ploy \log(d_p/ \alpha)$ \\

\hline
\end{tabular}
\end{center}
\caption{\textbf{Theoretical analysis of aggregation schema} $\alpha = M/N$ is the fraction of the Byzantine workers.$d_p$ is the size of prediction dimension,$d$ is the size of the gradient or parameters dimension.$\sigma$ is the varaince of one dimension}
\label{tab:theory_analysis}
\end{table*}


\section{Attacks on Aggregation Schemes}\label{attacks}

In this section we detail the attacks proposed in the literature on different aggregation schemes used for federated learning.
We also introduce two new attacks, one targeting the MwuAverage (Section. \ref{aggregation:mwu}) and similar aggregations .

% and other targeting the DKKLMS-mean (Section. \ref{aggregation:dkklms_smm})


\subsection{Baseline attacks}


\subsubsection{Label flip poisoning}\label{attack:lf_poison}

Hayes et al. \cite{hayes2018contamination} propose a simple poisoning attack where adversary flips the labels of her local training data in a particular fashion to poison it.
We call this attack \emph{label flip poisoning} attack.
As the adversary controls up to $M$ malicious clients, the label flipping strategy is consistent across all the $M$ clients.
Then the $M$ clients use the poisoned data to learn their local model, $\theta_i$, and share corresponding updates with the central server.
We use this simple attack as one of the baseline attacks.






\subsubsection{Naive poisoning}\label{attack:naive_poison}

The threat model (Section. \ref{ps:threat_model}) considers an omniscient adversary who can observe all the benign updates.
Therefore, the second baseline attack we use to evaluate different aggregation schemes crafts the malicious update to be arbitrarily far from the average of benign updates.
The malicious update, $\theta_m$, is then shared by each malicious client with the central server.
In \eqref{naive_poison}, $\theta'$ is a vector with arbitrarily large values and is of the same dimensions as any $\theta_i$.

\begin{equation}\label{naive_poison}
\theta_m = \frac{\sum^n_{i=1} \theta_i}{n} + \theta' \qquad n=(N-M)
\end{equation}











\subsection{Strategic poisoning attack}




\subsubsection{Little is enough attack(LIE)}\label{attack:lie}

Baruch et al. \cite{baruch2019a} propose an attack called \emph{little is enough} .
The attack is aims to circumvent defenses similar to $TrimmedMean$, Bulyan and Krum (Section. \ref{aggregation:bulyan}) all of which assume that the adversary would craft the malicious predictions far from the benign predictions in order to maximize the effect on final models.
The intuition behind the attack is that small perturbations along all the $d$-dimensions of malicious update, $\theta^m$, should suffice to affect model's convergence and also circumvent the defenses.
The attack is described in Algorithm. \ref{alg:lie}.



\begin{algorithm}
\caption{LIE Attack \cite{baruch2019a}}
\label{alg:lie}
\begin{algorithmic}[1]
\State \textbf{Input}: Benign updates $\mathcal{P}\leftarrow(\theta_1,...,\theta_{N-M})$, $N$, $M$
\State Number of required workers for majority:
\vspace{-.3em}
$$s=\floor{\frac{N}{2}+1}-M$$
\vspace{-.3em}
\State Using $z$-table, set $z=\underset{z}{max}\Big(\phi(z)<\frac{N-s}{N}\Big)$
\For {$j \in [d]$}
	\State Calculate mean, $\mu_j$, and covariance, $\sigma_j$ of $\mathcal{P}$
	\State $\theta_m^j\leftarrow \mu_j+z\sigma_j$
\EndFor
\State Append $M$ malicious updates, $\theta_m$, to $\mathcal{P}$
\State \textbf{Output}: $\mathcal{P}$
\end{algorithmic}
\end{algorithm}



Our experiments show that, along with Bulyan and Krum aggregation schemes, the LIE attack works also against the DKKLMS-mean aggregation (Section. \ref{aggregation:dkklms_smm}) used with federated learning (Algorithm. \ref{alg:fedavg}).


\subsection{Our attacks}






\subsubsection{Attack on schemes with averaging}\label{attack:attack_on_averaging}



We propose an attack that targets the three important aggregation schemes: MWU with averaging \cite{arora2012the}, CRH framework \cite{li2014resolving}.
The threat model considers an omniscient adversary that can observe all the benign updates and craft malicious updates.
The malicious updates are then shared with the central server through the malicious clients controlled by the adversary.


In a given epoch, the aforementioned aggregation schemes assign weights to a client based on the distance of her update from \emph{weighted average} of the updates of all clients.
The attack exploits the fact that, all clients are given equal weight to start with.
The intuition therefore is if adversary inserts a malicious update at a large distance from the average of benign updates, in the first epoch, it will shift the average by arbitrary amount.
Now, the adversary only needs to insert an update equal to the new malicious average.
This way, at the end of first epoch, negligible weights are assigned to all the benign clients and the first malicious update, and the weight of second malicious update will be close to 1.
This way, utility of the aggregate in each epoch can be completely jeopardized.

The adversary only needs two malicious clients with the two updates crafted as \eqref{at_on_avg}; here $n$ is the number of benign clients in the collaboration.

\begin{align}\label{at_on_avg}
\theta^1_m &= \frac{\sum^n_{i=1} \theta_i}{n} + \theta' \\
\theta^2_m &= \frac{\sum^n_{i=1} \theta_i+\theta^1_m}{n+1}
\end{align}










\subsubsection{PCA attack}\label{attack:pca_attack}





The second attack, we propose, targets the aggregation schemes that filter malicious points in the data by projecting the data on its principal axes.
Specifically, we target the DKKLMS-mean \ref{aggregation:dkklms_smm} aggregation.
However, the attack will work on any aggregation scheme that filters malicious points in the space of principal axes \cite{lai2016agnostic,li2018principled,diakonikolas2017being}.
We call it \emph{PCA} attack, because the attack analyzes the principal components of given data to craft the malicious update.
Assume some data, $D$, with $\mathbf{V}$ as the matrix of eigenvectors; eigenvectors are along the column of $\mathbf{V}$.
Then the projected data, called \emph{principal components}, of $D$ is given by $PC = \mathbf{V}.D$.
$PC$ can be reverted back to $D$ as : $D=\mathbf{V}^{T}.PC$, where $\mathbf{V}^{T}$ is transpose of $\mathbf{V}$.
This property allows PCA attack to craft the malicious update along principal axes and project it back.



The intuition behind the attack is similar to that of LIE attack \ref{attack:lie}.
The attack computes principal components of benign updates and then crafts the malicious update, $\theta_{pc}^m$, similar to the LIE attack.
$\theta_{pc}^m$ is then projected back simply by: $\theta^m = \mathbf{V}^T.\theta_{pc}^m$.
PCA attack is described in Algorithm \ref{alg:pca}




\begin{algorithm}
\caption{PCA attack}
\label{alg:pca}
\begin{algorithmic}[1]
\State \textbf{Input}: Benign updates $\mathcal{P}\leftarrow(\theta^1,...,\theta^{N-M})$, $N$, $M$

\State $\mathbf{V} \leftarrow$ eigenvectors of $\mathcal{P}$

\State $PC \leftarrow \mathbf{V}.\mathcal{P}$
\Comment Compute principal components of data

\State $\theta_{pc}^m \leftarrow \text{LIE}(PC)$
\Comment Mount LIE attack in the principal axes space

\State $\theta^m \leftarrow \mathbf{V}^T.\theta_{pc}^m$
\State Append $M$ malicious updates, $\theta^m$, to $\mathcal{P}$
\State \textbf{Output}: $\mathcal{P}$
\end{algorithmic}
\end{algorithm}





PCA attack works well against DKKLMS-mean as we show in our experiments.
Furthermore, only LIE attack also prevents the federated model from converging is DKKLMS-mean aggregation scheme is used.





\section{Cronus}
In the federated learning, the clients send the local knowledge to the server and the server aggregate the knowledge from all local clients and return it back to the local machine.
For the existing work, the common representation of the knowledge is the model gradient or the model parameters.
There are three foundational limitations to share the knowledge via the model gradient or the parameter: (1) Sharing the high dimensional parameter or gradients (2) The aggregation algorithm error guarantee is dependent on the data dimension. (3)\red{Leakage the privacy information of the local model. Even the local model only share the parameter or the gradient, the adversary still can observe the gradient or parameter and infer the private data through the membership attack}


In order to fix this problem, we proposed Cronus as a variant of federate learning. In our protocol, we improve the existing algorithm from two aspects: (1) Transfer knowledge via the output of the model. (2) Apply high-dimensional robust mean estimation.

\subsection{Share Knowledge via Prediction}
Our first strategy takes the output of the local models to transfer knowledge. Instead of using the model's parameters or gradients, we share the prediction vector of local models on the public data. In this case, the Byzantine worker can only affect the result through the prediction which limited the power of the adversary.




\begin{algorithm}
\caption{\textbf{\red{Cronus learning}}:  $X_p$ is public dataset
}\label{cronus_learning}
\begin{algorithmic}[1]
\Procedure {\textsf{\small{ClientOp}}}{$X_p,\hat{Y}_{agg}$}
\State $D_p = \{X_p,\hat{Y}_{agg}\}$
\For{T epochs}
\State $\theta_i \leftarrow$ \textsc{\textsf{\small{TrainAdv}}}($\theta_i, D_i$)
	\State $\theta_i \leftarrow$ \textsc{\textsf{\small{Train}}}($\theta_i, D_p$)
\EndFor


\State $\hat{Y}_{i} = \theta(X_p)$

\State return $\hat{Y}_{i}$ to server

\EndProcedure

\Procedure {\textsf{\small{ServerOp}}}{$ \hat{Y}_{0},\hat{Y}_{1},..,\hat{Y}_{n}$}
% \State Wait for and collect all $\Delta\theta_i$ from clients.
\State $\hat{Y}_{agg} = f_\textsf{\tiny{AGG\_CRONUS}}(\hat{Y}_{0},\hat{Y}_{1},...,\hat{Y}_{n})$ \hfill

\State return $\hat{Y}_{agg}$ to clients

\EndProcedure

\end{algorithmic}
\end{algorithm}


\noindent\textbf{\red{Training procedure}}

% The Cronus framework have $N$ clients to train the local model independently$\{\theta_1, \theta_2, ..., \theta_N\}$ on local dataset $\{D_1, D_2, ..., D_N\}$.

% Iniailly, the local model trained on the local dataset $D_{i}$


% and sends the prediction $\hat{y}_i$ on the public dataset $X_p$  to the server, preserving the local private training dataset and local private model parameters or gradients. The server receives the prediction vector from various local models, then aggregate the prediction $\hat{y}_{agg}$ and send to the local models. The local model update the model on the public data with the aggregated labels $\hat{y}_{agg}$ and the local dataset $D_i$.

The Cronus contains two training phase:
In Phase-1, all clients train their local model $\theta_i$, using adversarial regularization (\textsc{\textsf{\small{TrainAdv}}}) on the local dataset $D_{i}$ to get an acceptable level of accuracy and privacy against membership inference independently.
% There is no collaboration in Phase-1.
In Phase-2, clients share prediction vectors $\hat{Y}_i$ on $X_p$ with other via the aggregate algorithm on the server.

\begin{enumerate}
\item Each client shares predictions  $\hat{Y_i}$ from their model $\theta_i$ on the public dataset $X_p$ with the central curator.
\item Central curator calculates $\hat{Y}_{agg} =f_\textsf{\tiny{AGG\_CRONUS}}(\hat{Y}_i,..,\hat{Y}_N)$ and send the $\hat{Y}_{agg}$ to each clients.
\item Each client update the model $\theta_i$ on private data $D_i$, using \textsc{\textsf{\small{TrainAdv}}} and non-private $X_p,\hat{Y}_{agg}$ in the normal training way \textsc{\textsf{\small{Train}}}.
\end{enumerate}

Algorithm \ref{cronus_learning} describes the collaboration phase in detail.Initially, the client does not train on the public data since there is no aggregated label $\hat{Y}_{agg}$ for the public data. After the first iteration, the clients update the model on the public dataset with the aggregated label.

The intuition for prediction based knowledge sharing is that each client should benefit from the diversity and knowledge of other local models distilled through the aggregate predictions on $\hat{Y}_{agg}$, similar to the case of distillation and ensemble learning \cite{hinton2014distilling,breiman2001random}.
\red{At the same time, the adversarial regularization mitigates the membership inference risk.
Note that, in the end, there will not be a single global model, but individual clients with local models improved in terms of classification accuracy and resilience to the membership inference risk.
Therefore, all the client's models can be deployed as global models.}

\red{There are two advantages to share the knowledge via the prediction}
(1)Sharing the knowledge via the prediction of the public data reduces the dimension of the input for the aggregation algorithm, result in a better bound for the Byzantines error. (2) The prediction vector distribution follow concentrated distribution as we show in the \red{Figure..}. (3) \red{Sharing the prediction is black box access to the model which preserve more privcay comapred with white-box access.}
However, when the prediction vector of public data is large, the limitation of the high dimensional mean estimation still exits.
To solve the problem, we introduce the high dimensional mean estimation algorithm in Cronus framework.



\subsection{Robust Mean Estimation}
In the Cornus protocol, from the aggregation algorithm, the various knowledge learned from different training dataset can be shared. As shown in the last section, there are lots of work trying to estimate the mean via different aggregation schema. However,
through the Table ~\ref{tab:theory_analysis},we can see that the error guarantee of aggregation algorithm proposed in the related work is dependent on the dimension of the input. In the recent work \cite{diakonikolas2017being},
the aggregation algorithm is proposed for the high dimensional dataset.

\begin{theorem}\cite{diakonikolas2017being}
Let G be a sub-guassian distribution on $\mathbb{R}^d$ with mean vector $\mu$ and parameter $\nu = \Theta(1)$, mean vector $\mu^G$,covariance matrix $I$,and $\epsilon > 0 $. Let S be an $\epsilon-corrupted $ set of samples from G of size $\Omega((d/\epsilon^2)) ploy \log(d/\epsilon)$. There exists an efficient algorithm that, on input S and $\epsilon > 0$,returns a mean vector $\hat{\mu}$ so that with probability at least 9/10 we have $|| \hat{\mu} - \mu^G|| = O(\epsilon\sqrt{\log(1/\epsilon)})$
\end{theorem}

The key idea of the algorithm proposed in the \cite{diakonikolas2017being} is to filter the points which work together to change the empirical aggregation result instead of filtering each point independently. The real dataset should concentrate very well near the real mean of the distribution. If the aggregation result $\hat{u}$ is far away from the true mean $\mu$, then the adversary points must be the source of the deviation along the direction of the $\hat{\mu} - \mu$.
Based on the intuition, the method tries to project all the points onto the top eigenvector and throw away the points which are farthest away along with this projection. There are a few advantages when we apply this filtering algorithm:
\begin{enumerate}
    \item The error guarantee is independent of the dimension. Even when the dimension of prediction is large, the Cronus is still robust against the Byzantine adversary points.
    \item The sample complexity is dependent on the dimension. In our settings, each client contributes to one sample. To achieve the tight error guarantee, all we need to do is to increase the participant numbers.
    \item  All the steps in the algorithm can be done in nearly linear time.
\end{enumerate}


\begin{algorithm}
\caption{\red{Robust Mean Estimation \cite{diakonikolas2017being}}}
\label{alg:dkklms_smm}
\begin{algorithmic}[1]

\State \textbf{Input}: An $\epsilon$-corrupted set of the smaples S
\State Compute mean, $\mu_S$, and covariance matrix, $\Sigma_S$, of $S$
\State Compute approximations for the largest absolute eigenvalue $\lambda^*$ of $\Sigma_S$ and the associated unit eignvector $v^*$
\If {$||\Sigma_S||_2 \leq o(\epsilon \log1/\epsilon)$}
    \State \textbf{Output}: $\mu_S$
\EndIf
\State Let $\delta = 3\sqrt{\epsilon(||\Sigma||_2-1)}$
\State $Tail(T,d,\epsilon,\delta) = 8\exp(- T^2 /2 v) + 8 \frac{\epsilon}{T^2 \log(d\log(\frac{d}{\epsilon \delta}))}$
\State Find T > 0 such that \\

    $\Pr\limits_{X \in_{u} S'}[|v^* \dot (X - \mu^{S'})| > T + \delta] > Tail(T,d,\epsilon,\delta)$

\State \textbf{Output}: $\{x \in S': |v^* \dot (x - \mu^{S'})| \leq T + \delta\}$

\end{algorithmic}
\end{algorithm}

For the Cornus framework, the combination of the sharing the knowledge via prediction and the robust mean estimation help to obtain a better error guarantee as shown in Table ~\ref{tab:theory_analysis}



\red{Whether this algorithm should put in the experiements?}


Based on the practical modification mentioned in \cite{jerry2018robust}, we modify the theoretical algorithm as Algorithm \ref{alg:dkklms_smm} to apply it into our framework .

\begin{algorithm}
\caption{Mean estimation in Cronus: $f_\textsf{\tiny{AGG\_CRONUS}}$}
\label{alg:dkklms_smm}
\begin{algorithmic}[1]

\State \textbf{Input}: $S=(\hat{Y}_1,\hat{Y}_2...,\hat{Y}_N)$, $\epsilon$

\State Compute mean $\mu$, and covariance matrix $\Sigma$  of $S$
\State Find the eigenvector $v^*$ with highest eigenvalue $\lambda^*$ of $\Sigma$
\State $\tau(\hat{Y}_i)=|v^*.(\hat{Y}_i-\mu)|$
\State Let $c\in [0.5,1.5]$ be a parameter to be tuned
\State Let $T$ be the $1-c\epsilon$ percentile of $\{\tau(\hat{Y}_i):\hat{Y}_i \in S\}$
\State $S'=\{\hat{Y}_i \in S: \tau(\hat{Y}_i)<T\}$
\State \textbf{Output}: $median(S')$
\end{algorithmic}
\end{algorithm}

The aggregation algorithm gives us a good theoretical guarantee independent of the dimension of the input which can be applied for the various dataset.


\subsection{Performance analysis}
% \subsection{Communication cost analysis:}\label{comm_cost}




% Communication bandwidth is an important parameter of distributed learning because, different clients may have different bandwidth available at different times.
% In Cronus, the bandwidth corresponds to size of prediction matrix clients send to the central server.
% We employ various techniques to compress the predictions before sharing and empirically evaluate their effect on performance of final client models.
% Each client shares prediction logits in form of matrix of size $X\times Y$ where $X$ is subset of public data, $D_p$, and $Y$ is subset of total number of classes.
% Each logit is of size $b$-bits, therefore total communication bandwidth required to send predictions once is $(b \times X \times Y)$.
% Next, we describe the compression techniques employed and evaluated, and the corresponding communication cost.
% Table~\ref{comm_cost} represents communication costs associated with each technique.


% \subsubsection{Sharing compressed predictions.}
% For $i^{th}$ client, $\mathsf{\textsc{Clientop}}$, in Algorithm~\ref{cronus_learning}, returns $Y_{D_p,i}$ that has $y_{min}$ and $y_{max}$ as the minimum and maximum values respectively.
% Assuming a $b$-bit system, we first scale each $b$-bit logit, $y\in Y_{D_p,i}$, to $[0,r]$ range and discretize the range to be representable using $2^{b/c}$-bits.
% Then, Eq.\eqref{compress} gives expression to compresses $y$ to $\bar{y}$.
% Client $i$ has to send all such compressed predictions along with uncompressed $y_{min}$ and $y_{max}$ values for server to decompress; $[0,1]$ is public knowledge.
% Decompression of $\bar{y}$ is performed using Eq.~\eqref{decompress} where server chooses a $b$-bit number randomly from the range where $\bar{y}$ lies.


% \begin{equation}
% \label{compress}
% \bar{y}=\floor{(\frac{y-y_{min}}{y_{max}-y_{min}}).\frac{2^{b/c}}{r}}_{2^{b/c}-\text{bits}}
% \end{equation}

% \begin{multline}
% \label{decompress}
% y=\mathsf{rand}(\ [y_{min}+\frac{r}{2^{b/c}}\times \bar{y}\times (y_{max}-y_{min}),\\ y_{min}+\frac{r}{2^{b/c}}\times (\bar{y}+1)\times (y_{max}-y_{min})) \ )
% \end{multline}







% \subsubsection{Sharing predictions on subset of $D_p$.}
% In this method, communication is reduced by sharing predictions on a subset of public dataset.
% Each client randomly chooses $\bar{D}_p\subset D_p$ to share predictions for; we denote the fraction $\frac{\bar{D}_p}{ D_p}$ as $f$.
% Along with $Y_{\bar{D_p},i}$, $i^{th}$ client also shares indexes of samples in $\bar{D}_p$ wrt $D_p$.
% Consider $|D_p|=10$; now if client shares prediction only for first sample, she will send index $[0]$ or if she shared prediction for first and fifth sample, indexes sent are $[0,4]$ and so on.
% Note that, these indexes incur $|D_p|$ bits of communication if sent as a one-hot vector.
% Indexes are required for aggregation at the server; while computing aggregate of $t^{th}$ sample, server considers predictions of all the clients with $t^{th}$ index set to 1.

% % \subsubsection{Sharing difference of predictions.}
% % % Shokri et al.~\cite{shokri2015privacy} propose to share difference between parameters of the updated model and the downloaded model.
% % In this method, on the client side, communication is reduced by sharing difference, $\Delta Y_{D_p}$, of predictions that are downloaded, $Y_{D_p}$, and that are obtained by $\mathsf{\textsc{Clientop}}$, $Y_{D_p,i}$.
% % We use a threshold, $\tau$, to decide if the difference is significant enough to share or not; in our experiments, we set $\tau$ as some small fraction of maximum value in $Y_{D_p,i}-Y_{D_p}$.
% % The client side compression is given by Eq.~\eqref{diff_decompress} where $\mathbb{I}_{\text{condition}}$ is indicator function that is 1 if condition is true and 0 otherwise and therefore, $\mathbb{I}_{[(Y_{D_p,i}-Y_{D_p})>\tau]}$ is a binary matrix representing whether a logit is significant or not and is of same size as $D_p$.

% % \begin{align}
% % \label{diff_compress}
% % \Delta Y_{D_p}&=\mathbb{I}_{[(Y_{D_p,i}-Y_{D_p})>\tau]}*(Y_{D_p,i}-Y_{D_p}) \\
% % \label{diff_decompress}
% % Y_{D_p,i}&=Y_{D_p}+\Delta Y_{D_p}
% % \end{align}




% % On the server side, aggregation is performed by simply adding $\Delta Y_{D_p}$ to $Y_{D_p}$ to get true $Y_{D_p,i}$ for $i^{th}$ client as given by Eq.~\eqref{diff_decompress}.
% % As the models converge, the predictions matrix $(|D_p|\times |C|)$ becomes sparser as $\Delta Y_{D_p}$ logits become insignificant which reduces the communication significantly.



% \subsubsection{Sharing top-$k$ predictions.}
% In this scheme, a client calculates confidence over classes for each sample in $D_P$ and shares top-$k$predictions for the sample based on these confidences; client shares predictions over entire $D_p$.
% We calculate confidence over classes by passing prediction vector of logits through a softmax layer.
% Along with $k$ top predictions, client shares bit-vectors corresponding to class indexes which incurs $|D_p|\times |C|$ bits of communication.
% On server side, server aggregates the predictions by combining the class indexes and predictions.
% The empirical evaluation of all the compression methods is in Section \ref{exp:comm_cost}.




\subsection{Computation complexity}


==> intro_exp_para.tex <==
% Using four benchmark datasets, we comprehensively compare the robustness of Cronus with traditional federated learning using important aggregation schemes from the literature.
\texbf{We evaluate the robustness of all the state-of-the-art aggregation algorithms when used in the conventional federated learning \cite{mhamdi2018the,blanchard2017machine,mcmahan2017communication,yin2018byzantine} against the strong poisoning attacks, and show their severe susceptibility to adversarial updates.}
For instance, malicious parties who mount the \emph{little is enough} attack \cite{baruch2019a} significantly reduce  the classification accuracy of models learned using state-of-the-art Bulyan and Krum aggregations \cite{mhamdi2018the,blanchard2017machine}: For CIFAR10 dataset from 89.0\% to 75.6\% and for SVHN dataset from 94.5\% to just 15.5\%.
We introduce a very effective poisoning attack against aggregations based on multiplicative weight updates \cite{arora2012the,li2014resolving} and show that it reduces the accuracy of  federated learning with such aggregation algorithms to close to random guessing, e.g., 10\% for CiFAR10.
However, \textbf{Cronus is secure against all these attacks due to its robust knowledge transfer.}
Due to the strongest attack on Cronus, the reduction in accuracy is 1.6\% for Purchase, is 1.3\% for SVHN, is 1.5\% for MNIST, and 4\% for CIFAR10.



Cronus allows parties with heterogeneous model architectures to participate in the collaboration.
We evaluate various aspects of this feature of Cronus using Purchase dataset.
We show that heterogeneous collaboration does not reduce the accuracy of party models compared to its homogeneous counterparts, e.g.,.



The Cronus learning also allows for local party models to prevent sensitive information leakage through their predictions by training the models using adversarial regularization \cite{nasr2018machine}, an optimal defense against membership inference attacks.
We note that the Cronus learning is robust even when such adversarial regularization is enabled by the parties during training.
For instance, the strongest poisoning attack on Cronus reduces the accuracy of adversarially regularized party models by just 0.7\%, i.e., from 79.2\% to 78.5\%.

